Learning Is a Kan Extension

Previous work has demonstrated that efficient algorithms exist for computing Kan extensions and that some Kan extensions have interesting similarities to various machine learning algorithms. This paper closes the gap by proving that all error minimisation algorithms may be presented as a Kan extension. This result provides a foundation for future work to investigate the optimisation of machine learning algorithms through their presentation as Kan extensions. A corollary of this representation of error-minimising algorithms is a presentation of error from the perspective of lossy and lossless transformations of data.

==> sections/loss.tex <==
\section{Loss}

\begin{definition}[Optimisation Problem]
\label{definition:optimisation}
\begin{align*}
Given \quad & Loss: D \rightarrow \mathbb{R}_+\quad &&\\
\textrm{minimise} \quad & Loss(x)&&
\end{align*}
\end{definition}

\begin{definition}[Positive Monoid]
A monoid $S$ is positive if for all $x,y \in S$ then \[xy = Id_* \implies x=Id_*\quad \wedge \quad y= Id_*\]
\end{definition}

\begin{definition}[Monoid Flavoured Preorder]
Given a positive monoid $S$ an $S$ flavoured preorder is a category $\Phi$ equipped with a functor $\leq : \Phi \rightarrow S$. Where for any two objects $x,y \in \Phi$ then $x\leq_S y$ if there exists a morphism $f : x \rightarrow y$ such that $\leq(f) = Id_*$
\end{definition}

%add explanation that morphism transitivity and associativity reproduce preorder axioms

\begin{definition}[Lower Bounded Preorder ]
A preorder $C$ is Lower bounded if there exists a bottom element $\bot$ such that for any other object $x \in C$ then $\bot \leq x$.
\end{definition}

\begin{definition}[Monoid Flavoured Preorder 2]
Given a monoidal preorder $S$, an $S$ flavoured preorder is a category $P$ equipped with a lax 2-functor $\Phi : P \rightarrow S$. For any two objects $x,y \in P$ then $x\leq_\Phi y$ if and only if there exists an $f : x \rightarrow y$ and $\sigma : \Phi(f) \Rightarrow \Phi(Id_*)$
\end{definition}

\begin{lemma}
Given a monoid flavoured preorder $\Phi : P \rightarrow S$ and $x,y,z \in P$, if there exists $g : x \rightarrow y$, $h : y \rightarrow z$, and $\sigma : \Phi(hg) \Rightarrow Id_*$ then $y \leq_\Phi z$.
\end{lemma}

\begin{proof}
By the definition of a Lax 2-Functor (Def \ref{definition:Lax2Functor}) there exists a 2-morphism $\gamma:\Phi(h)\Phi(g) \Rightarrow \Phi(hg)$
\end{proof}

\begin{proposition}[Adjunction Loss minimiser]
\label{prop:adjoint_min_band}
Given a bounded $S$ flavoured preorder $\leq : \Phi \rightarrow S$, and functor $Loss : D \rightarrow \Phi$ with left adjoint $L : \Phi \rightarrow D$, then $L(\bot)$ is a global minima of $Loss$.
\end{proposition}

\begin{proof}
By the definition of an adjunction (Def \ref{def:AdjointFunctorTriangle}), the adjunction unit, $\eta : Id_{\Phi} \Rightarrow Loss \circ L$ is a universal factorisor. Meaning that for any morphism $f : c \rightarrow Loss(d)$ there is a unique morphism $Loss(\tilde{f}) : Loss(L(c)) \rightarrow Loss(d)$ such that $Loss(\tilde{f})\eta_c = f$.

Set $c$ to be $\bot \in \Phi$. Because $\bot$ is the bottom object of the $S$ flavoured preorder $\Phi$ then for all $d \in D$, $\bot \leq_S Loss(d)$, implying that there exists a morphism $f : \bot \rightarrow Loss(d)$ such that $\leq(f) = Id_*$.

This then suggests that for all $d \in D$ there is a morphism $Loss(\tilde{f}) : Loss(L(\bot)) \rightarrow Loss(d)$ such that $Loss(\tilde{f})\eta_c =\ f$
\begin{align*}
Id_* &= \leq(f)=\ \leq(Loss(\tilde{f})\eta_c)=\ (\leq(Loss(\tilde{f})))(\leq(\eta_c))\\
&\implies \leq(Loss(\tilde{f})) = Id_*\\
&\implies Loss(L(\bot)) \leq_S Loss(d)
\end{align*}
Meaning that for all $d \in D$ that $Loss(L(\bot)) \leq_S Loss(d)$ making $L(\bot)$ a global minima of $Loss$.
\end{proof}

\begin{proposition}[Kan Loss Minimiser]
\label{prop:kan_min_band}
Given a bounded $S$ flavoured preorder $\leq : \Phi \rightarrow S$, and a functor $Loss : D \rightarrow \Phi$ the left Kan lift $Lift_{Loss}\ \bot(*)$, if it exists, is a global minima of $Loss$.
% https://q.uiver.app/#q=WzAsMyxbMSwwLCJEIl0sWzIsMSwiXFxQaGkiXSxbMCwxLCJcXG1hdGhiZnsxfSJdLFsyLDEsIlxcYm90IiwyXSxbMiwwLCJMaWZ0X3tMb3NzfVxcIFxcYm90IiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzAsMSwiTG9zcyJdLFszLDAsIlxcZXRhIiwyLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwfX1dXQ==
\[\begin{tikzcd}
	& D \\
	{\mathbf{1}} && \Phi
	\arrow["Loss", from=1-2, to=2-3]
	\arrow["{Lift_{Loss}\ \bot}", dashed, from=2-1, to=1-2]
	\arrow[""{name=0, anchor=center, inner sep=0}, "\bot"', from=2-1, to=2-3]
	\arrow["\eta"', shorten <=3pt, Rightarrow, from=0, to=1-2]
\end{tikzcd}\]
\end{proposition}

\begin{proof}
By the definition of a left Kan lift, there is a universal natural transform $\eta : \bot \Rightarrow Loss \circ (Lift_{loss}\ \bot)$ meaning that for any other lift $F : \mathbf{1} \rightarrow D$ with natural transform $\gamma : \bot \Rightarrow Loss \circ F$ there is a unique natural transform $\epsilon : (Lift_{loss}\ \bot) \Rightarrow F$ such that $ (Loss \cdot \epsilon)\eta = \gamma$. As $\mathbf{1}$ is the terminal category, given any element $d \in D$ one can produce an $F$ such that $F(*) = d$. Since, $\bot$ is the bottom element of $\Phi$ then $\bot \leq_S Loss(F(*))=Loss(d)$ implying that there exists an $f : \bot \rightarrow Loss(F(*))$ such that $\leq(f) = Id_*$. Construct $\gamma : \bot \rightarrow Loss\circ F$, using $f$ as its single morphism $\gamma_* = f$.

The existence of an $\epsilon$ corresponding to this $F$ and $\gamma$ implies a morphism $(Loss \cdot \epsilon)_* : Loss(Lift_{loss}\ \bot(*)) \rightarrow Loss(d)$ such that $(Loss \cdot \epsilon)_*\eta_* = \gamma_* = f$.
\begin{align*}
Id_* &= \leq(f) =\ \leq((Loss \cdot \epsilon)_*\eta_*) = \ \leq((Loss \cdot \epsilon)_*)\ \wedge\ \leq(\eta_*)\\
&\implies \leq((Loss \cdot \epsilon)_*) = Id_*\\
&\implies Loss(Lift_{Loss}\ \bot(*)) \leq_S Loss(d)
\end{align*}
Meaning that for all $d \in D$ that $Loss(Lift_{loss}\ \bot(*)) \leq_S Loss(d)$  making $Lift_{Loss}\ \bot(*)$ a global minima of $Loss$.
\end{proof}
